A Minimal Formulation of Session Types: The Sessions of Trios in Concert

Session types are a type-based approach to the verification of message-passing programs. They specify communication structures essential to enforcing program correctness; by relying on sequencing constructs, a session type can precisely describe the intended order of communication actions through a channel. In this paper we study a fragment of session types that makes a very limited use of sequencing; we call it minimal session types. In the context of a core process calculus with sessions and higher-order concurrency, we establish two technical results. First, we prove that every process P typable with standard session types can be compiled down into a process D(P) typable with minimal session types. Second, we prove that P and D(P) are behaviorally equivalent. These results show that having sequencing in both processes and session types is convenient, but that only sequencing in processes is truly indispensable, as it can correctly codify sequencing in types. Our developments draw inspiration from work by Parrow on behavior-preserving decompositions of untyped processes using trios, i.e., processes with exactly three nested prefixes. By casting Parrow's approach in the realm of typed processes, our developments reveal a conceptually simple formulation of session types, supported by static and dynamic correctness results.

==> sources/contributions_and_outline.tex <==

\paragraph{Contributions \& Outline.}
In summary, in this paper we present the following contributions:
\begin{enumerate}
\item We identify the class of \emph{minimal session types} (MST) as a simple fragment of standard session types for \HO without sequencing that retains its absolute expressiveness (\Cref{d:mtypesi}).
\item We show how to decompose standard session types into minimal session types, and how to decompose processes typable with standard session types into processes typable with minimal session types. This is a result of static correctness (\Cref{t:decompcore}).
\item We show that the decomposition of a process is behaviorally equivalent to the original process. This is a result of \emph{dynamic correctness}, formalized in terms of \emph{MST bisimulations}, a typed behavioral equivalence that we introduce here (\Cref{t:dyncorr}).
\item We develop optimizations and extensions of our decomposition that bear witness to its robustness.
\end{enumerate}
%
%
%
The rest of the paper is organized as follows.
In \secref{s:lang} we recall the preliminaries on the session type system for \HO, which is the core process calculus for session-based concurrency on which we base our developments.
In \secref{s:decomp} we present \emph{minimal session types}, and the decomposition of well-typed \HO processes into minimal session types processes, accompanied by explanations and examples.
In \secref{ss:dynamic} we show the correctness of the decomposition, by establishing an \emph{MST bisimulation} between an \HO process and its decomposition.
In \secref{s:opt} we examine two optimizations of the decomposition that are enabled by the higher-order nature of our setting.
In \secref{ss:exti} we discuss extensions of our approach to consider constructs for branching and selection.
Finally, in \secref{s:rw} we elaborate further on related work and in \secref{s:concl} we present some closing remarks.
\appendx{The appendix contains omitted definitions and proofs.}

\paragraph{Differences with the conference version.}
An earlier version of this paper was presented at ECOOP 2019~\cite{APV19}.
The current paper revises the conference version, includes further examples, and incorporates a major addition: \secref{ss:dynamic} on dynamic correctness, including the notion of an MST bisimulation and the constructed bisimulation relation,  is completely new to this presentation.

==> sources/dynamic-correctness-table-thesis.tex <==
\begin{table}[!t]
    \begin{tabular}{ |l|l|l|}
      \rowcolor{gray!25}
      \hline
      $P$ &
        \multicolumn{2}{l|}{
      \begin{tabular}{l}
        \noalign{\smallskip}
        $\Cb{\tilde W}{\tilde x}{P}$
        \smallskip
      \end{tabular} 
    } 
         \\
      \hline
    $Q_1 \parallel Q_2$ 
    &
      \begin{tabular}{l}
      \noalign{\smallskip}
         $\big\{ R_1 \parallel R_2: 
         R_1 \in \Cb{\tilde W_1}{\tilde y}{Q_1}, 
         R_2 \in \Cb{\tilde W_2}{\tilde w}{Q_2}
         \big\}$
         \smallskip 
      \end{tabular}
      &
      %side-conditions
      \begin{tabular}{l}
        \noalign{\smallskip}
        $\wtd y = \fv{Q_1}$, $\wtd w = \fv{Q_2}$ \\
        $\subst{\tilde W}{\tilde x} = 
        \subst{\tilde W_1}{\tilde y} \cdot \subst{\tilde W_2}{\tilde w}$ 
        \smallskip
      \end{tabular}
      \\
     \hline
    $\news{m:C}\,Q$~
    &
      \begin{tabular}{l}
      \noalign{\smallskip}
         $\left\{\news{\wtd m : \Gt{C}} \news{\tilde \prop^m}{\,R} : 
          R \in 
         \Cb{\tilde W}{\tilde x}{Q\sigma} \right\}$
         \smallskip 
        %  \\
        %  $\big\{\news{\wtd s : \mathcal{R}({\trec{t}{S}})}
        %           {\news{\prop^s}
        %           \news{\prop^{\dual s}}R} :
        %            R \in \Cb{\tilde W}{\tilde x}{Q\sigma} \big\}$ 
        %            \smallskip 
      \end{tabular}
      &
      %side-conditions
      \begin{tabular}{l}
        \noalign{\smallskip}
        $\widetilde m = (m_1,\ldots,m_{\len{\Gt{C}}})$
        \\
        $\sigma = \subst{m_1 \dual{m_1}}{m \dual{m}}$
        \\
        % $\wtd \prop^m = \prop^m \cdot \prop^{\dual m}$
        $\tilde \prop^m = \linecondit{\tr(C)}{\prop^m \cdot \prop^{\dual m}}{\epsilon}$
        \smallskip
      \end{tabular}
      \\
     \hline
    $Q$
    &
      \begin{tabular}{l}
      \noalign{\smallskip}
      $\big\{ \Rb{\tilde v} \Par \apropout{k}{\wtd B}  \Par \B{k}{\tilde x}{P} \}$
      \\  
              % $\cup \big\{ \Rb{\tilde v \setminus n} \Par 
              % \propout{k}{\wtd B}
              % % \binp{\prop^n}{b}(\appl{b}{\wtd n})
              % \Rb{n}
              % \Par \B{k}{\tilde x}{P} : n \in \rfn{P} \big\}$ 
              % \\ 
              $\cup$ 
            $\big\{ \Rb{\tilde v \setminus \tilde r} \Par R: 
            R \in \Db{\tilde W}{\tilde x}{P},~ 
            \wtd r = \rfni{R} \big\}$
            % $\big\{ \Rb{\tilde v} \Par \apropout{k}{\wtd B}  \Par \B{k}{\tilde x}{P},$
            % \\  
            %         $\Rb{\tilde v \setminus r} \Par \propout{k}{\wtd B}
            %         \binp{\prop^r}{b}(\appl{b}{\wtd r})
            %         \Par \B{k}{\tilde x}{P} \big\}$ 
            %         \\ 
            %         $\cup$ 
            %       $\big\{ \Rb{\tilde v \setminus \tilde r} \Par R: 
            %       R \in \Db{\tilde W}{\tilde x}{P},~ 
            %       \wtd r = \rfni{R} \big\}$
         \smallskip 
      \end{tabular}
      &
      %side-conditions
      \begin{tabular}{l}
        \noalign{\smallskip}
        $\wtd W \vrelate \wtd B$ \\ 
        % $r \in \rfn{P}$, 
        $\wtd v = \rfn{P\subst{\tilde W}{\tilde x}}$ 
        % $\wtd v = \rfn{P}$ 
        % \\
        % $R_3 \in $ \\ 
        % $\wtd r = \rfni{R_3}$ 
        % \\
        % $\wtd \prop_{i} = \fpn{R_i}, i \in \{1,2,3\}$
          % $\wtd W \vrelate \wtd B$ \\
          % $\wtd \prop = \fpn{R}$
        \smallskip
      \end{tabular}
      \\
     \hline
    $H$
    &
      \begin{tabular}{l}
      \noalign{\smallskip}
      % $\big\{ H' : H\subst{\tilde W}{\tilde x} 
      % \processrelate H'  \big\}$
      $\big\{ \Rb{\tilde v} \parallel H' : H\subst{\tilde W}{\tilde x} 
      \processrelate H'  \big\}$
      % $\{ H' : H\subst{\tilde W}{\tilde x} \processrelate H'\}$
        %  $\{ \news{\wtd \prop}H' : H\subst{\tilde W}{\tilde x} \processrelate H', 
        %  \wtd \prop = \fpn{H'} \}$
         \smallskip 
      \end{tabular}
      &
      %side-conditions
      \begin{tabular}{l}
        \noalign{\smallskip}
        $\tilde v= \rfn{H\subst{\tilde W}{\tilde x}}$
        % $\tilde v= \rfn{H}$
        \smallskip
      \end{tabular}
      \\
      \hline
      \hline
      \rowcolor{gray!25}
      $P$ &
        \multicolumn{2}{l|}{
      \begin{tabular}{l}
        \noalign{\smallskip}
        $\Db{\tilde W}{\tilde x}{P}$
        \smallskip
      \end{tabular}
    } 
    
    
    \\
      \hline
     
    
    $\bout{u_i}{V_1}Q$
    &
      \begin{tabular}{ll}
      \noalign{\smallskip}
      $\bullet~\lnot$$\tr(C)$: &
      \\
            \quad  $\big\{\bout{u_i}{V_2}
             \apropout{k}{\widetilde B_2} \Par 
        \B{k}{\tilde z}{Q\sigma} \big\}$ 
        % $\quad  V_1 \sigma \subst{\tilde W_1}{\tilde y} \vrelate V_2, 
        % \wtd W_2 \vrelate \wtd B_2 \}$
        & %(\text{if } $\lnot$$\tr(C)$)
        \smallskip
        \\
        \hdashline 
        \noalign{\smallskip}
        $\bullet~\tr(C)$: & 
        \\
              \quad $\big\{ \abbout{\prop^u}{M^{\tilde B_2}_{V_2}}   \Par$ 
              $\B{k}{\tilde w}{Q},\ 
               \appl{M^{\tilde B_2}_{V_2}}{\wtd u} \Par \B{k}{\tilde w}{Q},$ 
               & %(\text{if } $\tr(C)$)
               \\ 
              \qquad $ {\bbout{u_{\indT{S}}}{V_2}}{} 
              (\apropout{k} {\wtd B_2} \Par 
              \recprovx{u}{x}{\wtd u}
              % \binp{\prop^u}{b}(\appl{b}{\wtd u})
          ) 
          \Par \B{k}{\tilde w}{Q} \big\}$ 
          % \\
              % $: V_1 \subst{\tilde W_1}{\tilde y} \vrelate V_2,\ 
              % \wtd W_2 \vrelate \wtd B_2 \}$
              \smallskip
              \\
              \quad where:
              \\
              \quad\quad$M^{\tilde B}_V = \abs{\wtd z}
                {\bbout{z_{\indT{S}}}{V}}{}$  
                $(\apropout{k}{\wtd B} \Par 
                \recprovx{u}{x}{\wtd z}
                % \binp{\prop^u}{b} (\appl{b}{\wtd z})
            )$ 
            \smallskip
      \end{tabular}
      &
      %side-conditions
      \begin{tabular}{l}
        \noalign{\smallskip}
        $\wtd y = \fv{V_1}$, $\wtd w = \fv{Q}$ \\
        $\subst{\tilde W}{\tilde x} = 
        \subst{\tilde W_1}{\tilde y} \cdot \subst{\tilde W_2}{\tilde w}$ \\
        $\sigma = \subsqn{u_i}$ \\
        $V_1 \sigma \subst{\tilde W_1}{\tilde y} \vrelate V_2$ 
        \\ 
        $\wtd W_2 \vrelate \wtd B_2$ \\
        % $\wtd v = \rfn{\bout{u}{V}{Q}\subst{\tilde W}{\tilde x}}$ \\
        % $\wtd v = \rfn{P\subst{\tilde W}{\tilde x}}$ \\
        $\wtd z = (z_1,\ldots, z_{\len{\Rts{}{s}{S}}})$ \\
        $\wtd u = (u_1,\ldots, u_{\len{\Rts{}{s}{S}}})$ 
        % $\sigma = \begin{cases}
        %   \incrname{u}{i} & \text{if } u_i:S \\
        %   \epsilon & \text{otherwise}
        %   \end{cases}$ 
        \smallskip
      \end{tabular}
        \\
      \hline
      
      
    $\binp{u_i}{y}Q$
    &
      \begin{tabular}{ll}
      \noalign{\smallskip}
      $\bullet~\neg$$\tr(C)$: & 
      \\
             \quad $\big\{\binp{u_i}{y}\apropout{k}{\wtd By} 
             \Par 
             \B{k}{\tilde xy}{Q\sigma} \big\}$
             & %(\text{if } $\neg$$\tr(C)$)
        \smallskip 
        \\
        \hdashline 
        \noalign{\smallskip}
         $\bullet~\tr(C)$: & \\
                \quad $\big\{  \abbout{\prop^u}
                {M^{\tilde B}_y} 
                \Par \B{k}{\tilde xy}{Q},\
                 \appl{M^{\tilde B}_y}{\wtd u} \Par \B{k}{\tilde xy}{Q},$ 
                 & %(\text{if } $\tr(C)$)
                 \\
             \qquad  ${ \binp{u_{\indT{S}}}{y}
             (\apropout{k}{\wtd By} \Par 
             \recprovx{u}{x}{\wtd u}
              % \binp{\prop^u}{b}(\appl{b}{\wtd z})
              )
              \Par \B{k}{\tilde xy}{Q}} \big\}$ 
              % \\
                % $ : \wtd W \vrelate \wtd B \}$
                \\
                \quad where:
                \\
                \qquad $M^{\tilde B}_y = 
                \abs{\widetilde z}{\binp{z_{\indT{S}}}{y}
                (\apropout{k}{\wtd By} \Par 
                \recprovx{u}{x}{\wtd z}
                % \binp{\prop^u}{b}(\appl{b}{\wtd z})
                )}$
                \smallskip 
      \end{tabular}
      &
      %side-conditions
      \begin{tabular}{l}
        \noalign{\smallskip}
        $\wtd W \vrelate \wtd B$ \\
        $\sigma = \subsqn{u_i}$ \\
        % $\wtd v = \rfn{P\subst{\tilde W}{\tilde x}}$ \\
        % $\wtd v = \rfn{\binp{u_i}{y}Q\subst{\tilde W}{\tilde x}}$ \\
        $\wtd z = (z_1,\ldots,z_{\len{\Rts{}{s}{S}}})$ \\
        $\wtd u = (u_1,\ldots,u_{\len{\Rts{}{s}{S}}})$ 
        % $\sigma = \begin{cases}
        %   \incrname{u}{i} & \text{if } u_i:S \\
        %   \epsilon & \text{otherwise}
        %   \end{cases}$ 
        \smallskip 
      \end{tabular}
      \\
      \hline
    $\appl{V_1}{(\wtd r, u_i)}$
    &
      \begin{tabular}{l}
        \noalign{\smallskip}
        $\big \{   \overbracket{\prop^{r_{l}}!\big\langle 
        \lambda \wtd z_{l}. \prop^{r_{{l}+1}}!\langle\lambda \wtd z_{{l}+1}.\cdots. 
     \prop^{r_n}!\langle \lambda \widetilde z_n.}^{|\tilde r| - {l} +1} 
     Q_l \rangle \,\rangle \big\rangle, $  \\
     \quad $  \lambda \wtd z_l.
     \overbracket{
         \prop^{r_{l+1}}!\langle\lambda \wtd z_{l+1}.\cdots. 
     \prop^{r_n}!\langle \lambda \wtd z_n.}^{|\tilde r| - l} 
     Q_l \rangle \, \big\rangle \ {\wtd r_l},$ \\
     \qquad $: 1 \leq l \leq n,\ V_1\subst{\tilde W}{\tilde x} \vrelate V_2 \big \} $ \\
    $\cup\, \{\appl{V_2}{\wtd r_1, \ldots, \wtd r_n, \wtd m}
    : V_1\subst{\tilde W}{\tilde x} \vrelate V_2 \}$ \\
    where:
    \\
     \quad $Q_l = \appl{V_2}{(\wtd r_1,\ldots,\wtd r_{l-1}, \wtd z_{l}, \ldots, 
     \wtd z_n, \wtd m)}$
    \smallskip
      \end{tabular}
      &
      %side-conditions
      \begin{tabular}{l}
        \noalign{\smallskip}
        $\forall r_i \in \widetilde r.(r_i: S_i \wedge \mathsf{tr}(S_i) \wedge$\\
          \qquad $\wtd{z_i} = (z^i_1,\ldots,z^i_{\len{\Rts{}{s}{S_i}}}), $ \\
          \qquad $\wtd{r_i} = (r^i_1,\ldots,r^i_{\len{\Rts{}{s}{S_i}}}) )$\\
          % $\wtd v = \rfn{V\subst{\tilde W}{\tilde x}}$ \\
          $u_i : C$ \\ 
          $\wtd m = (u_i, \ldots, u_{i+\len{\Gt{C}}-1})$
          \smallskip
      \end{tabular}
        \\
      \hline
    $Q_1 \Par Q_2$
    &
      \begin{tabular}{l}
      \noalign{\smallskip}
         $\big\{ \propout{k}{\wtd B_1}
         \apropout{k+l}{\wtd B_2} \Par \B{k}{\tilde y}{Q_1}
          \Par 
         \B{k+l}{\tilde z}{Q_2} \big\} $ \\
        %  $\quad \wtd W_1 \vrelate \wtd B_1$, $\wtd W_2 \vrelate \wtd B_2  \}$ \\ 
         $\cup$ \\
         $ \big\{(R_1 \Par R_2) : R_1 \in
         \Cb{\tilde W_1}{\tilde y}{Q_1}, R_2 \in 
         \Cb{\tilde W_2}{\tilde z}{Q_2} \big\}$ 
         \smallskip 
      \end{tabular}
      &
      %side-conditions
      \begin{tabular}{l}
        \noalign{\smallskip}
          $l = \plen{Q_1}$, $\wtd W_1 \vrelate \wtd B_1$, $\wtd W_2 \vrelate \wtd B_2$ \\
        $\wtd y = \fv{Q_1}$, $\wtd z = \fv{Q_2}$  \\
        $\subst{\tilde W}{\tilde x} = \subst{\tilde W_1}{\tilde y} \cdot \subst{\tilde W_2}{\tilde z}$
        \smallskip 
      \end{tabular}
      \\ 
      \hline 
    $\inact$
    &
      \begin{tabular}{l}
      \noalign{\smallskip}
         $\inact$ 
         \smallskip 
      \end{tabular}
      &
      %side-conditions
      \begin{tabular}{l}
        \noalign{\smallskip}
        \smallskip 
      \end{tabular}
      \\
      \hline
    \end{tabular}
    
    \caption{The sets $\Cb{\tilde W}{\tilde x}{P}$ and $\Db{\tilde W}{\tilde x}{P}$. \label{mst:t:tablecd}}
    \end{table} 

==> sources/introduction.tex <==
Session types are a type-based approach to the verification of message-passing programs.
A session type specifies what and when should be exchanged through a channel.
This makes session types a useful tool to enforce safety and liveness properties related to communication correctness.
Originated in the realm of concurrency theory, session types have had a significant impact on the foundations of programming languages~\cite{DBLP:journals/csur/HuttelLVCCDMPRT16}, but also on their practice~\cite{DBLP:journals/ftpl/AnconaBB0CDGGGH16}.
Our goal in this work is to understand to what extent session types can admit simpler, more fundamental formulations.
This foundational question has concrete practical ramifications, as we discuss next.

In session-typed languages, \emph{sequencing} constructs in types and processes specify the intended structure of message-passing protocols.
For example, in the session type $S = \btinp{\mathsf{int}} \btinp{\mathsf{int}} \btout{\mathsf{bool}} \tinact$, sequencing (denoted `$;$') allows us to specify a protocol for a channel that \emph{first} receives (?)
two integers, \emph{then} sends (!)
a boolean, and \emph{finally} ends.
As such, $S$ could type a service that checks for integer equality.
Sequencing in types goes hand-in-hand with sequencing in processes, which is specified using prefix constructs (denoted~`$.$').
The $\pi$-calculus process $P = \binp{s}{x_1} \binp{s}{x_2} \bout{s}{x_1=x_2} \inact$ is an implementation of the equality service: it \emph{first} expects two values on name $s$, \emph{then} outputs a boolean on $s$, and \emph{finally} stops.
Thus, name $s$ in $P$ conforms to the session type~$S$.
Session types can also specify sequencing within labeled choices and recursion; these typed constructs are also in close match with their respective process expressions.

Session types have been originally developed as a typing discipline for $\pi$-calculus for the analysis of message-passing protocols between exactly two parties~\cite{honda.vasconcelos.kubo:language-primitives}.
Since then session types have been extended in many directions.
We find, for instance, multiparty session types~\cite{HYC08}, and extensions with dependent types, assertions, exceptions, and time (cf.~\cite{DL10,DBLP:journals/csur/HuttelLVCCDMPRT16} for surveys).
All these extensions seek to address natural research questions on the expressivity and applicability of session types theories.

Here we address a different, if opposite, question: \emph{is there a minimal formulation of session types?}
This is an appealing question from a theoretical perspective, but seems particularly relevant to the practice of session types: identifying the ``core'' of session types could enable their integration in languages whose type systems do not have certain advanced constructs present in session types, such as sequencing.
For instance, the Go programming language offers primitive support for message-passing concurrency; it comes with a static verification mechanism which can only enforce that messages exchanged along channels correspond with their declared payload types---it cannot ensure essential correctness properties associated with the ordering of messages and the structure of the protocols.
This observation has motivated the development of advanced static verification tools based on session types for Go programs; see, e.g.,~\cite{DBLP:conf/cc/NgY16,DBLP:conf/icse/LangeNTY18}.


This paper identifies and studies the properties of an elementary formulation of session types, which we call \emph{minimal session types}.
Minimal session types are session types without sequencing. 
That is, in
session types such as `$\btout{U} S$' and `$\btinp{U} S$', we stipulate that $S$ can only correspond to $\tinact$, the type of the terminated protocol.

Adopting minimal session types entails dispensing with sequencing, which is arguably the most distinctive feature of session types.
While this may appear as a far too drastic restriction, it turns out that it is not:
we show that for every process $P$ typable under standard (non minimal) session types, there is a  \emph{decomposition} of $P$, denoted $\D{P}$, a process that 
codifies the sequencing information given by the session types (protocols) of $P$ using additional synchronizations, extracted from its protocols.
\Cref{f:idea} illustrates the key idea of the decomposition using the process $P$ and session type $S$ motivated above. 
Because $P$ contains three actions in sequence (as stipulated by $S$), its decomposition  $\D{P}$ consists of three processes in parallel---each of them implementing one action of $P$---as well as of mechanisms for orchestrating these parallel processes: the synchronizations on names $c_2, \ldots, c_5$ ensure that the sequencing in $P$ is preserved and that received names are properly propagated. These three parallel processes are typable with minimal session types (in the figure, they are given below each process), which are obtained by suitably ``slicing'' $S$.

Our main finding is that $\D{P}$ satisfies two important properties: first, it is well-typed using minimal session types (\emph{static correctness}); second, it is behaviorally equivalent to $P$ (\emph{dynamic correctness}).
These properties ensure that having sequencing in both types and processes is convenient but \emph{redundant}: only sequencing at the level of processes is truly indispensable.


\begin{figure}[!t]
\begin{mdframed}
		\begin{center}
		\hspace*{0.2cm} 
		\begin{tikzpicture}[scale=1.75]
		\tikzstyle{ann} = [draw=none,fill=none,right]
		\pgfmathsetmacro{\h}{0.0}
		\pgfmathsetmacro{\a}{-2.5}
		\pgfmathsetmacro{\d}{-1.3}

			\node[draw,dotted](A) at (\h, 0) {$P = \binp{s}{x_1}\binp{s}{x_2}\bout{s}{x_1 = x_2} \inact$};
			\node[draw=none] at (\h,-0.45) {$s : {?({\mathsf{int}})}; {?({\mathsf{int}})};
		 {!\langle {\mathsf{bool}}\rangle};\tinact$};
			\node[draw,dotted] (B) at (\h, \d) {$\D{P}$};
			\draw[->, thick] (\h,-0.575 - 0.2) -- (\h,\d+0.3);
			\node[draw,dotted] (T1) at (\h-3.0,\a) {$\cbpropinp{2}{}\binp{s_1}{x_1}\cbapropout{3}{x_1}$};
			\node at (\h-1.5,\a) {$\parallel$};
			\node[draw,dotted] (T2) at (\h,\a) {$\cbpropinp{3}{y_1}\binp{s_2}{x_2}\cbapropout{4}{y_1, x_2}$}; 
			\node at (\h+1.45, \a) {$\parallel$};
			\node[draw,dotted] (T3) at (\h+3.0,\a) {$\cbpropinp{4}{x_1, x_2}\bout{s_3}{x_1 = x_2}\cbapropout{5}{}$};
			\node at (\h-3.0,\a-0.45) {$s_1:{?({\mathsf{int}})};\tinact$};
			\node at (\h-3.0,\a-0.75) {$\prop_2:{?()};\tinact$};
			\node at (\h,\a-0.45) {$s_2:{?({\mathsf{int}})};\tinact$};
			\node at (\h,\a-0.75) {$\prop_3:{?({\mathsf{int}})};\tinact$};
%			\node at (0,-4.10) {$\prop_4:\textcolor{red}{?}\blue{\mathsf{int}};\tinact$};
			\node at (\h+3.0,\a-0.45) {$s_3:{!\langle{\mathsf{bool}}\rangle};\tinact$};
			\node at (\h+3.0,\a-0.75) {$\prop_4:{?({\mathsf{int}, \mathsf{int}})};\tinact$};
			\draw[->, color=magenta, thick](\h-2.5,\a+0.25) edge[bend left] node [left] {} (\h-1,\a+0.25);
			\draw[->, color=magenta, thick](\h+0.5,\a+0.25) edge[bend left] node [left] {} (\h+2,\a+0.25);
			\node[draw=none] {};
			\draw[->, color=magenta, thick] (B) edge[bend right=22] node [left] {} (T1); 
			%\draw[->, dotted, thick] (B) edge (T2);
			\draw[<-, color=magenta, thick] (B) edge[bend left=22] node [left] {} (T3); 
		\end{tikzpicture}
		\end{center}
		\end{mdframed}
\caption{The process decomposition, illustrated. Arrows in \textcolor{magenta}{magenta} indicate synchronizations orchestrated by the decomposition $\D{P}$. \label{f:idea}}
		\end{figure}
		

The definition of $\D{P}$ is interesting on its own, as it draws inspiration from a known result by Parrow~\cite{DBLP:conf/birthday/Parrow00}, who showed that any \emph{untyped} $\pi$-calculus process can be decomposed as a collection of \emph{trio processes}, i.e., processes with at most three nested prefixes~\cite{DBLP:conf/birthday/Parrow00}.

The question of how to relate session types with other type systems has attracted interest in the past.
Session types have been encoded into, for instance, generic types~\cite{DBLP:journals/corr/GayGR14} and linear types~\cite{DBLP:conf/concur/DemangeonH11,DBLP:conf/ppdp/DardhaGS12,DBLP:journals/iandc/DardhaGS17}.
As such, these prior studies concern the \emph{relative expressiveness} of session types, where the expressivity of session types stands with respect to that of some other type system.
In sharp contrast, we study the \emph{absolute expressiveness} of session types: how session types can be explained in terms of themselves.
To our knowledge, this is the first study of its kind. %, and may open up new avenues for foundational and practical research.


Session types have been developed on top of different process languages (mainly, dialects of the $\pi$-calculus), and so choosing the target language for minimal session types is an important decision in our developments.
In this paper, our target language is \HO, the core process calculus for session-based concurrency studied by Kouzapas et al.~\cite{DBLP:conf/esop/KouzapasPY16,KouzapasPY17}.
\HO is a very small language, which only supports passing of abstractions (i.e., functions from names to processes) and lacks name-passing and recursion.
Nonetheless, \HO is very expressive, because both features can be encoded in \HO in a fully abstract way.
Moreover, \HO has a well-developed theory of behavioral equivalences~\cite{KouzapasPY17}. 
The combination of minimal number of features and expressivity makes \HO an excellent candidate for studying a minimal formulation of session types.
Indeed, as we will see, several aspects of our decomposition take advantage of the higher-order nature of  \HO.
%
Being a higher-order language, \HO is very different from the (untyped, first-order) $\pi$-calculus considered by Parrow~\cite{DBLP:conf/birthday/Parrow00}. 
% Also, the session types of \HO severely constrain the range and kind of conceivable decompositions.
Therefore, our technical results arise in a context very different from Parrow's.

% \input{contributions_and_outline.tex}


\paragraph{Contributions \& Outline.}
In summary, in this paper we present the following contributions:
\begin{enumerate}
\item We identify the class of \emph{minimal session types} (MST) as a simple fragment of standard session types for \HO without sequencing that retains its absolute expressiveness (\Cref{d:mtypesi}).
\item We show how to decompose standard session types into minimal session types, and how to decompose processes typable with standard session types into processes typable with minimal session types. This is a result of static correctness (\Cref{t:decompcore}).
\item We show that the decomposition of a process is behaviorally equivalent to the original process. This is a result of \emph{dynamic correctness}, formalized in terms of \emph{MST bisimulations}, a typed behavioral equivalence that we introduce here (\Cref{t:dyncorr}).
\item We develop optimizations and extensions of our decomposition that bear witness to its robustness.
\end{enumerate}
%
%
%
The rest of the paper is organized as follows.
In \secref{s:lang} we recall the preliminaries on the session type system for \HO, which is the core process calculus for session-based concurrency on which we base our developments.
In \secref{s:decomp} we present \emph{minimal session types}, and the decomposition of well-typed \HO processes into minimal session types processes, accompanied by explanations and examples.
In \secref{ss:dynamic} we show the correctness of the decomposition, by establishing an \emph{MST bisimulation} between an \HO process and its decomposition.
In \secref{s:opt} we examine two optimizations of the decomposition that are enabled by the higher-order nature of our setting.
In \secref{ss:exti} we discuss extensions of our approach to consider constructs for branching and selection.
Finally, in \secref{s:rw} we elaborate further on related work and in \secref{s:concl} we present some closing remarks.
\appendx{The appendix contains omitted definitions and proofs.}

\paragraph{Differences with the conference version.}
An earlier version of this paper was presented at ECOOP 2019~\cite{APV19}.
The current paper revises the conference version, includes further examples, and incorporates a major addition: \secref{ss:dynamic} on dynamic correctness, including the notion of an MST bisimulation and the constructed bisimulation relation,  is completely new to this presentation.

\paragraph{Colors.}
Throughout the paper we use different colors (such as \textcolor{\colorpro}{pink}  and \textcolor{\colortyp}{green}) to improve readability.
However, the usage of colors is not indispensable, and the paper can be followed in black-and-white.

==> sources/type_system.tex <==
\begin{figure}[t!]
	\begin{mdframed}
	\[
		\begin{array}{c}
		\inferrule[(Sess)]{}{\Gamma; \emptyset; \set{u:S} \proves u \hastype S} 
			\qquad
			\inferrule[(Sh)]{}{\Gamma \cat u : U; \emptyset; \emptyset \proves u \hastype U}
			\\ \\ 
			\inferrule[(LVar)]{}{\Gamma; \set{x: \lhot{C}}; \emptyset \proves x \hastype \lhot{C}}
							\qquad
			\inferrule[(RVar)]{}{\Gamma \cat \rvar{X}: \Delta; \emptyset; \Delta  \proves \rvar{X} \hastype \Proc}
					\\  \\
			\inferrule[(Abs)]{
				\Gamma; \Lambda; \Delta_1 \proves P \hastype \Proc
				\quad
				\Gamma; \es; \Delta_2 \proves x \hastype C
			}{
				\Gamma\backslash x; \Lambda; \Delta_1 \backslash \Delta_2 \proves \abs{{x}}{P} \hastype \lhot{{C}}
			}
			\quad
			\inferrule[(App)]{
				%\begin{array}{c}
					%U = \hot{C} \lor \shot{C}
					%\\
					{\Gamma; \Lambda; \Delta_1 \proves V \hastype \ghot{C} ~~
					\leadsto\, \in \{\lollipop, \sharedop\} \quad
					\Gamma; \es; \Delta_2 \proves u \hastype C
					}
			%	\end{array}
			}{
				\Gamma; \Lambda; \Delta_1 \cat \Delta_2 \proves \appl{V}{u} \hastype \Proc
			} 
	
			\\  \\
			\inferrule[(Prom)]{
				\Gamma; \emptyset; \emptyset \proves V \hastype 
							 \lhot{C}
			}{
				\Gamma; \emptyset; \emptyset \proves V \hastype 
							 \shot{C}
			} 
			\quad
			\inferrule[(EProm)]{
			\Gamma; \Lambda \cat x : \lhot{C}; \Delta \proves P \hastype \Proc
			}{
				\Gamma \cat x:\shot{C}; \Lambda; \Delta \proves P \hastype \Proc
			}
					\quad
			\inferrule[(End)]{
				\Gamma; \Lambda; \Delta  \proves P \hastype T \quad u \not\in \dom{\Gamma, \Lambda,\Delta}
			}{
				\Gamma; \Lambda; \Delta \cat u: \tinact  \proves P \hastype \Proc
			}
			\\  \\
			\inferrule[(Rec)]{
				\Gamma \cat \rvar{X}: \Delta; \emptyset; \Delta  \proves P \hastype \Proc
			}{
				\Gamma ; \emptyset; \Delta  \proves \recp{X}{P} \hastype \Proc
			}
			\qquad
				\inferrule[(Par)]{
				\Gamma; \Lambda_{i}; \Delta_{i} \proves P_{i} \hastype \Proc \quad i=1,2
			}{
				\Gamma; \Lambda_{1} \cat \Lambda_2; \Delta_{1} \cat \Delta_2 \proves P_1 \Par P_2 \hastype \Proc
			}
			\qquad
					\inferrule[(Nil)]{ }{\Gamma; \emptyset; \emptyset \proves \inact \hastype \Proc}
			\\  \\
			\inferrule[(Req)]{
			\begin{array}{c}
			\Gamma; \Lambda; \Delta_1 \proves P \hastype \Proc
			\quad
			\Gamma; \es; \es \proves u \hastype	\chtype{U}
			\\
			\Gamma; \es; \Delta_2 \proves V \hastype U		
				\end{array}
			}{
				\Gamma; \Lambda; \Delta_1 \cat \Delta_2 \proves \bout{u}{V} P \hastype \Proc
			}
			~~
%			\\ \\
%--
%			~~
			\inferrule[(Acc)]{
				\begin{array}{c}
					\Gamma; \Lambda_1; \Delta_1 \proves P \hastype \Proc
					\quad 
					\Gamma; \emptyset; \emptyset \proves u \hastype \chtype{U} 
					\\
					\Gamma; \Lambda_2; \Delta_2 \proves x \hastype U
					   \end{array}
			}{
				\Gamma\backslash x; \Lambda_1 \backslash \Lambda_2; \Delta_1 \backslash \Delta_2 \proves \binp{u}{x} P \hastype \Proc
			}	
			\\  \\
			\inferrule[(Send)]{
						%\begin{array}{c}
						u:S \in \Delta_1 \cat \Delta_2 %\\
						\quad
				\Gamma; \Lambda_1; \Delta_1 \proves P \hastype \Proc
				\quad
				\Gamma; \Lambda_2; \Delta_2 \proves V \hastype U
				%\end{array}
			}{
				\Gamma; \Lambda_1 \cat \Lambda_2; ((\Delta_1 \cat \Delta_2) \setminus u:S) \cat u:\btout{U} S \proves \bout{u}{V} P \hastype \Proc
			}
			\\  \\
								\inferrule[(Rcv)]{
			%\begin{array}{c}
				\Gamma; \Lambda_1; \Delta_1 \cat u: S \proves P \hastype \Proc
				\quad
				\Gamma; \Lambda_2; \Delta_2 \proves {x} \hastype {U}
			%	\end{array}
			}{
				\Gamma \backslash x; \Lambda_1\backslash \Lambda_2; \Delta_1\backslash \Delta_2 \cat u: \btinp{U} S \vdash \binp{u}{{x}} P \hastype \Proc
			}
\\ \\ 
			% 		\inferrule[(Bra)]{
			% 	 \forall i \in I \quad \Gamma; \Lambda; \Delta \cat u:S_i \proves P_i \hastype \Proc
			% }{
			% 	\Gamma; \Lambda; \Delta \cat u: \btbra{l_i:S_i}_{i \in I} \proves \bbra{u}{l_i:P_i}_{i \in I}\hastype \Proc
			% }
			% \qquad
			%  \inferrule[(Sel)]{
			% 	\Gamma; \Lambda; \Delta \cat u: S_j  \proves P \hastype \Proc \quad j \in I
			% }{
			% 	\Gamma; \Lambda; \Delta \cat u:\btsel{l_i:S_i}_{i \in I} \proves \bsel{u}{l_j} P \hastype \Proc
			% }
			% \\  \\
			\inferrule[(ResS)]{
				\Gamma; \Lambda; \Delta \cat s:S_1 \cat \dual{s}: S_2 \proves P \hastype \Proc \quad S_1 \dualof S_2
			}{
				\Gamma; \Lambda; \Delta \proves \news{s} P \hastype \Proc
			}
			\qquad
			\inferrule[(Res)]{
				\Gamma\cat a:\chtype{S} ; \Lambda; \Delta \proves P \hastype \Proc
			}{
				\Gamma; \Lambda; \Delta \proves \news{a} P \hastype \Proc
			}
			\end{array}
	\]
	\end{mdframed}
	%\vspace{-3mm}
	\caption{Typing Rules for $\HO$. 
	% (including selection and branching constructs).
	%See \appref{app:types} for a full account.
	\label{fig:typerulesmys}}
	%\Hline
	%\vspace{-1mm}
	\end{figure}
	%\myparagraph{Typing System of \HOp}
